Local Asymptotic Equivalence of the Bai and Ng (2004) and Moon and Perron (2004) Frameworks for Panel Unit Root Testing

This paper considers unit-root tests in large n and large T heterogeneous panels with cross-sectional dependence generated by unobserved factors. We reconsider the two prevalent approaches in the literature, that of Moon and Perron (2004) and the PANIC setup proposed in Bai and Ng (2004). While these have been considered as completely different setups, we show that, in case of Gaussian innovations, the frameworks are asymptotically equivalent in the sense that both experiments are locally asymptotically normal (LAN) with the same central sequence. Using Le Cam's theory of statistical experiments we determine the local asymptotic power envelope and derive an optimal test jointly in both setups. We show that the popular Moon and Perron (2004) and Bai and Ng (2010) tests only attain the power envelope in case there is no heterogeneity in the long-run variance of the idiosyncratic components. The new test is asymptotically uniformly most powerful irrespective of possible heterogeneity. Moreover, it turns out that for any test, satisfying a mild regularity condition, the size and local asymptotic power are the same under both data generating processes. Thus, applied researchers do not need to decide on one of the two frameworks to conduct unit root tests. Monte-Carlo simulations corroborate our asymptotic results and document significant gains in finite-sample power if the variances of the idiosyncratic shocks differ substantially among the cross sectional units.

==> graphs/sizesCombBICAnHet1_0.4_0.4_BN__Uniform.tex <==
\begin{table}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}S[table-figures-decimal=0,table-figures-integer=3]S[table-figures-decimal=0,table-figures-integer=3]S[table-figures-decimal=1,table-figures-integer=1]cSSScSSScSSS@{}}
\toprule
&&&&\multicolumn{3}{c}{i.i.d.}&&\multicolumn{3}{c}{AR(1)}&&\multicolumn{3}{c}{MA(1)}\\ \cmidrule{5-7} \cmidrule{9-11} \cmidrule{13-15}
{$n$} & {$T$} & {$\sqrt{\omega^4/\phi^4}$} & {} & {$\tUMP$} & {$\tUMPEMP$} & {$P_b$} & {} & {$\tUMP$} & {$\tUMPEMP$} & {$P_b$} & {} & {$\tUMP$} & {$\tUMPEMP$} & {$P_b$} \\
\midrule
25.0000 & 25.0000 & 0.6000 &  & 0.6250 & 2.6958 & 3.1833 &  & 1.8500 & 4.6667 & 4.1917 &  & 2.2028 & 6.8583 & 5.6139 \\
25.0000 & 50.0000 & 0.6000 &  & 1.4375 & 4.8000 & 4.1042 &  & 1.8167 & 5.2542 & 3.7417 &  & 3.0167 & 9.0833 & 6.0972 \\
25.0000 & 100.0000 & 0.6000 &  & 1.8500 & 5.5792 & 4.7625 &  & 2.3583 & 6.2208 & 4.2000 &  & 3.8167 & 10.2417 & 6.7556 \\
50.0000 & 50.0000 & 0.6000 &  & 2.0042 & 4.2917 & 3.5917 &  & 2.5750 & 4.5958 & 3.6250 &  & 5.2306 & 9.9861 & 6.6056 \\
50.0000 & 100.0000 & 0.6000 &  & 2.5667 & 4.9875 & 4.1750 &  & 2.9667 & 5.4458 & 3.7792 &  & 6.1250 & 10.9806 & 7.1833 \\
50.0000 & 200.0000 & 0.6000 &  & 3.0292 & 5.7208 & 4.5625 &  & 3.1917 & 5.6458 & 3.9083 &  & 5.1083 & 9.0861 & 6.0361 \\
100.0000 & 100.0000 & 0.6000 &  & 3.1583 & 4.8417 & 3.9625 &  & 3.2833 & 4.9208 & 3.7792 &  & 9.3778 & 13.4083 & 8.2778 \\
100.0000 & 200.0000 & 0.6000 &  & 3.4875 & 5.0667 & 4.4833 &  & 3.4708 & 5.1042 & 3.8583 &  & 6.8833 & 9.8000 & 6.4750 \\
100.0000 & 400.0000 & 0.6000 &  & 3.7208 & 5.3667 & 4.5667 &  & 4.4042 & 6.1292 & 4.6208 &  & 4.8556 & 7.0639 & 5.2250 \\
25.0000 & 25.0000 & 0.8000 &  & 0.8167 & 2.9833 & 3.4917 &  & 1.8417 & 4.2500 & 4.8125 &  & 2.3556 & 6.6000 & 6.4889 \\
25.0000 & 50.0000 & 0.8000 &  & 1.8292 & 4.9958 & 4.4625 &  & 1.8458 & 4.4083 & 4.1500 &  & 3.1361 & 8.3083 & 7.1083 \\
25.0000 & 100.0000 & 0.8000 &  & 2.2542 & 5.8875 & 5.4875 &  & 2.0042 & 4.8458 & 4.2625 &  & 4.0250 & 9.4444 & 8.0083 \\
50.0000 & 50.0000 & 0.8000 &  & 2.3792 & 4.7375 & 4.1417 &  & 2.3083 & 4.1625 & 4.2333 &  & 5.2500 & 9.3778 & 8.3417 \\
50.0000 & 100.0000 & 0.8000 &  & 3.0625 & 5.5583 & 5.0125 &  & 2.7333 & 4.7417 & 4.2625 &  & 5.9694 & 10.1889 & 8.5389 \\
50.0000 & 200.0000 & 0.8000 &  & 3.2042 & 5.7042 & 5.1333 &  & 3.1042 & 5.3083 & 4.7833 &  & 4.8667 & 8.1944 & 7.0028 \\
100.0000 & 100.0000 & 0.8000 &  & 3.5500 & 5.2792 & 4.6292 &  & 3.0125 & 4.3833 & 4.4125 &  & 8.8583 & 12.6056 & 10.6056 \\
100.0000 & 200.0000 & 0.8000 &  & 3.8292 & 5.4375 & 5.0583 &  & 3.4167 & 4.8208 & 4.6708 &  & 6.5306 & 9.1833 & 7.9361 \\
100.0000 & 400.0000 & 0.8000 &  & 4.0000 & 5.6042 & 5.2417 &  & 3.6875 & 5.2042 & 4.8167 &  & 4.7111 & 6.5278 & 5.8806 \\
25.0000 & 25.0000 & 1.0000 &  & 0.9542 & 3.3917 & 4.0792 &  & 1.9611 & 4.4278 & 5.3778 &  & 2.4500 & 6.6389 & 7.2917 \\
25.0000 & 50.0000 & 1.0000 &  & 1.8292 & 5.0583 & 4.9042 &  & 1.7667 & 4.3028 & 4.5194 &  & 3.1972 & 8.0750 & 8.1861 \\
25.0000 & 100.0000 & 1.0000 &  & 2.5625 & 5.8750 & 5.6750 &  & 2.1389 & 5.0667 & 5.0889 &  & 3.9778 & 8.8944 & 8.9306 \\
50.0000 & 50.0000 & 1.0000 &  & 2.5583 & 4.8167 & 4.6083 &  & 2.2361 & 3.8389 & 4.6861 &  & 5.1722 & 9.3250 & 10.1917 \\
50.0000 & 100.0000 & 1.0000 &  & 3.2667 & 5.5917 & 5.3958 &  & 2.7556 & 4.6722 & 5.0472 &  & 5.5778 & 9.6861 & 9.5083 \\
50.0000 & 200.0000 & 1.0000 &  & 3.6458 & 5.8958 & 5.7708 &  & 2.9833 & 5.0583 & 5.0917 &  & 4.9500 & 8.2583 & 8.2528 \\
100.0000 & 100.0000 & 1.0000 &  & 3.5958 & 5.3208 & 4.8875 &  & 2.9583 & 4.2542 & 5.0333 &  & 8.5000 & 11.9806 & 12.2389 \\
100.0000 & 200.0000 & 1.0000 &  & 3.9708 & 5.6875 & 5.4542 &  & 3.2417 & 4.5458 & 4.8542 &  & 6.3806 & 8.7417 & 8.8000 \\
100.0000 & 400.0000 & 1.0000 &  & 3.9292 & 5.6125 & 5.4208 &  & 3.7958 & 5.2708 & 5.4125 &  & 4.7667 & 6.5111 & 6.5611 \\
\midrule\multicolumn{3}{c}{Mean abs. dev. from 5\%}  &  &2.292 &0.61867 &0.5946 &  &2.2701 &0.4767 &0.58827 &  &1.3939 &4.0759 &2.709\\
\bottomrule
\end{tabular}}
\caption{Sizes (in percent) of nominal 5\% level tests  with heterogeneous alternatives where $U_i$ is drawn from a Uniform(0.2,1.8) distribution. Based on 36000 replications. Andrews Bandwidth.}
\label{table:sizesAnHet1_0.4_0.4_BN__Uniform}
\end{table}


==> graphs/sizesCombBICNeHet1_0.4_0.4_BN__Uniform.tex <==
\begin{table}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}S[table-figures-decimal=0,table-figures-integer=3]S[table-figures-decimal=0,table-figures-integer=3]S[table-figures-decimal=1,table-figures-integer=1]cSSScSSScSSS@{}}
\toprule
&&&&\multicolumn{3}{c}{i.i.d.}&&\multicolumn{3}{c}{AR(1)}&&\multicolumn{3}{c}{MA(1)}\\ \cmidrule{5-7} \cmidrule{9-11} \cmidrule{13-15}
{$n$} & {$T$} & {$\sqrt{\omega^4/\phi^4}$} & {} & {$\tUMP$} & {$\tUMPEMP$} & {$P_b$} & {} & {$\tUMP$} & {$\tUMPEMP$} & {$P_b$} & {} & {$\tUMP$} & {$\tUMPEMP$} & {$P_b$} \\
\midrule
25.0000 & 25.0000 & 0.6000 &  & 0.3417 & 1.1125 & 1.4583 &  & 1.3708 & 3.5792 & 3.7625 &  & 0.9361 & 3.3111 & 3.6972 \\
25.0000 & 50.0000 & 0.6000 &  & 0.6042 & 2.5708 & 2.3667 &  & 1.5542 & 4.4208 & 3.2542 &  & 1.2333 & 4.0444 & 3.2306 \\
25.0000 & 100.0000 & 0.6000 &  & 1.3625 & 4.2917 & 3.7250 &  & 2.2917 & 6.2750 & 4.0083 &  & 2.2111 & 6.4694 & 4.4778 \\
50.0000 & 50.0000 & 0.6000 &  & 0.8292 & 2.0042 & 1.7875 &  & 2.1750 & 3.9208 & 3.1958 &  & 1.7861 & 3.7667 & 3.0139 \\
50.0000 & 100.0000 & 0.6000 &  & 1.8000 & 3.8167 & 3.0750 &  & 2.9292 & 5.5125 & 3.6375 &  & 3.1722 & 5.9889 & 4.2472 \\
50.0000 & 200.0000 & 0.6000 &  & 2.4917 & 4.7000 & 3.6583 &  & 3.2708 & 5.7625 & 3.6125 &  & 2.6750 & 5.0361 & 3.6306 \\
100.0000 & 100.0000 & 0.6000 &  & 2.3167 & 3.5792 & 2.6708 &  & 3.3750 & 5.0625 & 3.6250 &  & 4.1083 & 6.1306 & 4.2361 \\
100.0000 & 200.0000 & 0.6000 &  & 2.7833 & 4.2708 & 3.4750 &  & 3.6708 & 5.3792 & 3.6000 &  & 3.2472 & 4.6556 & 3.3722 \\
100.0000 & 400.0000 & 0.6000 &  & 3.2667 & 4.8458 & 3.8833 &  & 4.2792 & 6.2000 & 4.2375 &  & 3.0444 & 4.5472 & 3.4611 \\
25.0000 & 25.0000 & 0.8000 &  & 0.3792 & 1.2458 & 1.6625 &  & 1.3708 & 3.2708 & 4.1875 &  & 1.0611 & 3.0833 & 4.2222 \\
25.0000 & 50.0000 & 0.8000 &  & 0.9250 & 2.8667 & 2.5208 &  & 1.5458 & 3.8125 & 3.6167 &  & 1.4139 & 3.9167 & 3.7444 \\
25.0000 & 100.0000 & 0.8000 &  & 1.7000 & 4.7000 & 4.2792 &  & 1.9167 & 4.8542 & 4.1625 &  & 2.4333 & 6.0417 & 5.1528 \\
50.0000 & 50.0000 & 0.8000 &  & 1.1125 & 2.4125 & 2.0875 &  & 1.9708 & 3.6250 & 3.6458 &  & 2.0528 & 3.6444 & 3.6250 \\
50.0000 & 100.0000 & 0.8000 &  & 2.1875 & 4.3458 & 3.5875 &  & 2.7625 & 4.8583 & 4.1375 &  & 3.1611 & 5.7000 & 4.8139 \\
50.0000 & 200.0000 & 0.8000 &  & 2.6708 & 4.8125 & 4.1208 &  & 3.1417 & 5.5125 & 4.4500 &  & 2.7111 & 4.6889 & 3.8556 \\
100.0000 & 100.0000 & 0.8000 &  & 2.5500 & 4.0417 & 3.1042 &  & 3.0792 & 4.4958 & 4.2917 &  & 4.0278 & 5.9194 & 5.3278 \\
100.0000 & 200.0000 & 0.8000 &  & 3.2458 & 4.7333 & 3.7000 &  & 3.5375 & 5.0417 & 4.3417 &  & 2.9889 & 4.3667 & 3.7444 \\
100.0000 & 400.0000 & 0.8000 &  & 3.6250 & 5.2000 & 4.4125 &  & 3.6417 & 5.1208 & 4.3375 &  & 3.1167 & 4.3667 & 3.6889 \\
25.0000 & 25.0000 & 1.0000 &  & 0.5042 & 1.4042 & 1.9292 &  & 1.4806 & 3.3472 & 4.6583 &  & 1.1333 & 3.1833 & 4.6194 \\
25.0000 & 50.0000 & 1.0000 &  & 0.9083 & 2.8542 & 2.6958 &  & 1.5028 & 3.6944 & 3.9083 &  & 1.4222 & 3.7778 & 4.1667 \\
25.0000 & 100.0000 & 1.0000 &  & 2.0417 & 4.6625 & 4.3125 &  & 2.1083 & 4.9944 & 4.9333 &  & 2.3944 & 5.7722 & 5.6167 \\
50.0000 & 50.0000 & 1.0000 &  & 1.4042 & 2.6208 & 2.3417 &  & 1.9250 & 3.3056 & 4.0139 &  & 1.9611 & 3.7694 & 4.4167 \\
50.0000 & 100.0000 & 1.0000 &  & 2.3958 & 4.3125 & 3.7333 &  & 2.7944 & 4.7056 & 4.8250 &  & 3.0167 & 5.2556 & 5.1333 \\
50.0000 & 200.0000 & 1.0000 &  & 3.0417 & 5.1417 & 4.5792 &  & 3.0833 & 5.1042 & 4.6958 &  & 2.8111 & 4.6639 & 4.3944 \\
100.0000 & 100.0000 & 1.0000 &  & 2.7542 & 4.0292 & 3.0583 &  & 3.0542 & 4.5000 & 4.7792 &  & 3.9139 & 5.5806 & 5.7583 \\
100.0000 & 200.0000 & 1.0000 &  & 3.3417 & 4.9250 & 3.9625 &  & 3.2625 & 4.7458 & 4.5042 &  & 2.9361 & 4.1111 & 3.8444 \\
100.0000 & 400.0000 & 1.0000 &  & 3.5542 & 5.1833 & 4.5042 &  & 3.6708 & 5.1792 & 4.8542 &  & 2.9944 & 4.2917 & 3.9639 \\
\midrule\multicolumn{3}{c}{Mean abs. dev. from 5\%}  &  &2.9949 &1.3099 &1.7892 &  &2.3791 &0.70442 &0.87865 &  &2.4828 &0.91502 &0.94527\\
\bottomrule
\end{tabular}}
\caption{Sizes (in percent) of nominal 5\% level tests  with heterogeneous alternatives where $U_i$ is drawn from a Uniform(0.2,1.8) distribution. Based on 36000 replications. Newey Bandwidth.}
\label{table:sizesNeHet1_0.4_0.4_BN__Uniform}
\end{table}


==> graphs/stamps/NpowersNeiidBN0.611.tex <==
\begin{figure}[ht]\footnotesize\begin{subfigure}[b]{0.3466\textwidth}\input{graphs/stamps/NpowersNe25_25_1_0.6_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/NpowersNe50_25_1_0.6_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/NpowersNe100_25_1_0.6_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\\ \begin{subfigure}[b]{0.3466\textwidth}\input{graphs/stamps/NpowersNe50_50_1_0.6_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/NpowersNe100_50_1_0.6_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/NpowersNe200_50_1_0.6_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\\ \begin{subfigure}[b]{0.3466\textwidth}\input{graphs/stamps/NpowersNe100_100_1_0.6_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/NpowersNe200_100_1_0.6_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/NpowersNe400_100_1_0.6_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\\ \begin{subfigure}[b]{\textwidth}\centering\input{graphs/stamps/lNpowersNe400_100_1_0.6_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\normalsize\caption{\label{NpowersNeiidBN0.611}Size-corrected power of unit-root tests as a function of $-h$ for varying sample sizes in the PANIC framework with i.i.d.\ factor innovations and i.i.d.\ idiosyncratic parts and $\sqrt{\omega^4/\phi^4}=0.6$. Based on \num{100000} replications.}\end{figure}

==> graphs/stamps/NpowersNeiidBN111.tex <==
\begin{figure}[ht]\footnotesize\begin{subfigure}[b]{0.3466\textwidth}\input{graphs/stamps/NpowersNe25_25_1_1_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/NpowersNe50_25_1_1_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/NpowersNe100_25_1_1_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\\ \begin{subfigure}[b]{0.3466\textwidth}\input{graphs/stamps/NpowersNe50_50_1_1_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/NpowersNe100_50_1_1_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/NpowersNe200_50_1_1_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\\ \begin{subfigure}[b]{0.3466\textwidth}\input{graphs/stamps/NpowersNe100_100_1_1_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/NpowersNe200_100_1_1_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/NpowersNe400_100_1_1_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\\ \begin{subfigure}[b]{\textwidth}\centering\input{graphs/stamps/lNpowersNe400_100_1_1_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\normalsize\caption{\label{NpowersNeiidBN111}Size-corrected power of unit-root tests as a function of $-h$ for varying sample sizes in the PANIC framework with i.i.d.\ factor innovations and i.i.d.\ idiosyncratic parts and $\sqrt{\omega^4/\phi^4}=1$. Based on \num{100000} replications.}\end{figure}

==> graphs/stamps/NpowersStatNeiidBN0.811DifMP.tex <==
\begin{figure}[ht]\footnotesize\begin{subfigure}[b]{0.36\textwidth}\input{graphs/stamps/NpowersStatNe25_25_1_0.8_iid_0.4_overdiffiid_0.4_MP_DifMP.tex}\end{subfigure}\begin{subfigure}[b]{0.32\textwidth}\input{graphs/stamps/NpowersStatNe50_25_1_0.8_iid_0.4_overdiffiid_0.4_MP_DifMP.tex}\end{subfigure}\begin{subfigure}[b]{0.32\textwidth}\input{graphs/stamps/NpowersStatNe100_25_1_0.8_iid_0.4_overdiffiid_0.4_MP_DifMP.tex}\end{subfigure}\\ \begin{subfigure}[b]{0.36\textwidth}\input{graphs/stamps/NpowersStatNe50_50_1_0.8_iid_0.4_overdiffiid_0.4_MP_DifMP.tex}\end{subfigure}\begin{subfigure}[b]{0.32\textwidth}\input{graphs/stamps/NpowersStatNe100_50_1_0.8_iid_0.4_overdiffiid_0.4_MP_DifMP.tex}\end{subfigure}\begin{subfigure}[b]{0.32\textwidth}\input{graphs/stamps/NpowersStatNe200_50_1_0.8_iid_0.4_overdiffiid_0.4_MP_DifMP.tex}\end{subfigure}\\ \begin{subfigure}[b]{0.36\textwidth}\input{graphs/stamps/NpowersStatNe100_100_1_0.8_iid_0.4_overdiffiid_0.4_MP_DifMP.tex}\end{subfigure}\begin{subfigure}[b]{0.32\textwidth}\input{graphs/stamps/NpowersStatNe200_100_1_0.8_iid_0.4_overdiffiid_0.4_MP_DifMP.tex}\end{subfigure}\begin{subfigure}[b]{0.32\textwidth}\input{graphs/stamps/NpowersStatNe400_100_1_0.8_iid_0.4_overdiffiid_0.4_MP_DifMP.tex}\end{subfigure}\\ \begin{subfigure}[b]{\textwidth}\centering\input{graphs/stamps/lNpowersStatNe400_100_1_0.8_iid_0.4_overdiffiid_0.4_MP_DifMP.tex}\end{subfigure}\normalsize\caption{\label{DifMPNpowersStatNeiidBN0.811}Difference between powers in the MP vs the PANIC framework as a function of $-h$ with overdiffiid factor innovations and i.i.d.\ idiosyncratic parts and $\sqrt{\omega^4/\phi^4}=0.8$. Based on \num{201000} replications.}\end{figure}

==> graphs/stamps/NpowersStatiidBN0.811DifMP.tex <==
\begin{figure}[ht]\footnotesize\begin{subfigure}[b]{0.36\textwidth}\input{graphs/stamps/NpowersStat25_25_1_0.8_iid_0.4_overdiffiid_0.4_MP_DifMP.tex}\end{subfigure}\begin{subfigure}[b]{0.32\textwidth}\input{graphs/stamps/NpowersStat50_25_1_0.8_iid_0.4_overdiffiid_0.4_MP_DifMP.tex}\end{subfigure}\begin{subfigure}[b]{0.32\textwidth}\input{graphs/stamps/NpowersStat100_25_1_0.8_iid_0.4_overdiffiid_0.4_MP_DifMP.tex}\end{subfigure}\\ \begin{subfigure}[b]{0.36\textwidth}\input{graphs/stamps/NpowersStat50_50_1_0.8_iid_0.4_overdiffiid_0.4_MP_DifMP.tex}\end{subfigure}\begin{subfigure}[b]{0.32\textwidth}\input{graphs/stamps/NpowersStat100_50_1_0.8_iid_0.4_overdiffiid_0.4_MP_DifMP.tex}\end{subfigure}\begin{subfigure}[b]{0.32\textwidth}\input{graphs/stamps/NpowersStat200_50_1_0.8_iid_0.4_overdiffiid_0.4_MP_DifMP.tex}\end{subfigure}\\ \begin{subfigure}[b]{0.36\textwidth}\input{graphs/stamps/NpowersStat100_100_1_0.8_iid_0.4_overdiffiid_0.4_MP_DifMP.tex}\end{subfigure}\begin{subfigure}[b]{0.32\textwidth}\input{graphs/stamps/NpowersStat200_100_1_0.8_iid_0.4_overdiffiid_0.4_MP_DifMP.tex}\end{subfigure}\begin{subfigure}[b]{0.32\textwidth}\input{graphs/stamps/NpowersStat400_100_1_0.8_iid_0.4_overdiffiid_0.4_MP_DifMP.tex}\end{subfigure}\\ \begin{subfigure}[b]{\textwidth}\centering\input{graphs/stamps/lNpowersStat400_100_1_0.8_iid_0.4_overdiffiid_0.4_MP_DifMP.tex}\end{subfigure}\normalsize\caption{\label{DifMPNpowersStatiidBN0.811}Difference between powers in the MP vs the PANIC framework as a function of $-h$ with overdiffiid factor innovations and i.i.d.\ idiosyncratic parts and $\sqrt{\omega^4/\phi^4}=0.8$. The factor is stationary.  Based on \num{201000} replications.}\end{figure}

==> graphs/stamps/NpowersiidBN0.611.tex <==
\begin{figure}[ht]\footnotesize\begin{subfigure}[b]{0.3466\textwidth}\input{graphs/stamps/Npowers25_25_1_0.6_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/Npowers50_25_1_0.6_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/Npowers100_25_1_0.6_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\\ \begin{subfigure}[b]{0.3466\textwidth}\input{graphs/stamps/Npowers50_50_1_0.6_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/Npowers100_50_1_0.6_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/Npowers200_50_1_0.6_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\\ \begin{subfigure}[b]{0.3466\textwidth}\input{graphs/stamps/Npowers100_100_1_0.6_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/Npowers200_100_1_0.6_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/Npowers400_100_1_0.6_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\\ \begin{subfigure}[b]{\textwidth}\centering\input{graphs/stamps/lNpowers400_100_1_0.6_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\normalsize\caption{\label{NpowersiidBN0.611}Size-corrected power of unit-root tests as a function of $-h$ for varying sample sizes in the PANIC framework with i.i.d.\ factor innovations and i.i.d.\ idiosyncratic parts and $\sqrt{\omega^4/\phi^4}=0.6$. Based on \num{100000} replications.}\end{figure}

==> graphs/stamps/NpowersiidBN0.811Dif.tex <==
\begin{figure}[ht]\footnotesize\begin{subfigure}[b]{0.3466\textwidth}\input{graphs/stamps/Npowers25_25_1_0.8_iid_0.4_iid_0.4_MP_Dif.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/Npowers50_25_1_0.8_iid_0.4_iid_0.4_MP_Dif.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/Npowers100_25_1_0.8_iid_0.4_iid_0.4_MP_Dif.tex}\end{subfigure}\\ \begin{subfigure}[b]{0.3466\textwidth}\input{graphs/stamps/Npowers50_50_1_0.8_iid_0.4_iid_0.4_MP_Dif.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/Npowers100_50_1_0.8_iid_0.4_iid_0.4_MP_Dif.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/Npowers200_50_1_0.8_iid_0.4_iid_0.4_MP_Dif.tex}\end{subfigure}\\ \begin{subfigure}[b]{0.3466\textwidth}\input{graphs/stamps/Npowers100_100_1_0.8_iid_0.4_iid_0.4_MP_Dif.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/Npowers200_100_1_0.8_iid_0.4_iid_0.4_MP_Dif.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/Npowers400_100_1_0.8_iid_0.4_iid_0.4_MP_Dif.tex}\end{subfigure}\\ \begin{subfigure}[b]{\textwidth}\centering\input{graphs/stamps/lNpowers400_100_1_0.8_iid_0.4_iid_0.4_MP_Dif.tex}\end{subfigure}\normalsize\caption{\label{DifNpowersiidBN0.811}(Size-corrected) power gains from using $\tUMPEMP$ over $P_b$ for varying values of $\sqrt{\omega^4/\phi^4}$ and sample sizes in the BN framework. Based on 500 replications.}\end{figure}

==> graphs/stamps/NpowersiidBN0.811DifMP.tex <==
\begin{figure}[ht]\footnotesize\begin{subfigure}[b]{0.3466\textwidth}\input{graphs/stamps/Npowers25_25_1_0.8_iid_0.4_iid_0.4_MP_DifMP.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/Npowers50_25_1_0.8_iid_0.4_iid_0.4_MP_DifMP.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/Npowers100_25_1_0.8_iid_0.4_iid_0.4_MP_DifMP.tex}\end{subfigure}\\ \begin{subfigure}[b]{0.3466\textwidth}\input{graphs/stamps/Npowers50_50_1_0.8_iid_0.4_iid_0.4_MP_DifMP.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/Npowers100_50_1_0.8_iid_0.4_iid_0.4_MP_DifMP.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/Npowers200_50_1_0.8_iid_0.4_iid_0.4_MP_DifMP.tex}\end{subfigure}\\ \begin{subfigure}[b]{0.3466\textwidth}\input{graphs/stamps/Npowers100_100_1_0.8_iid_0.4_iid_0.4_MP_DifMP.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/Npowers200_100_1_0.8_iid_0.4_iid_0.4_MP_DifMP.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/Npowers400_100_1_0.8_iid_0.4_iid_0.4_MP_DifMP.tex}\end{subfigure}\\ \begin{subfigure}[b]{\textwidth}\centering\input{graphs/stamps/lNpowers400_100_1_0.8_iid_0.4_iid_0.4_MP_DifMP.tex}\end{subfigure}\normalsize\caption{\label{DifMPNpowersiidBN0.811}(Size-corrected) power gains from using $\tUMPEMP$ over $P_b$ for varying values of $\sqrt{\omega^4/\phi^4}$ and sample sizes in the BN framework. Based on 10500 replications.}\end{figure}

==> graphs/stamps/NpowersiidBN111.tex <==
\begin{figure}[ht]\footnotesize\begin{subfigure}[b]{0.3466\textwidth}\input{graphs/stamps/Npowers25_25_1_1_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/Npowers50_25_1_1_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/Npowers100_25_1_1_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\\ \begin{subfigure}[b]{0.3466\textwidth}\input{graphs/stamps/Npowers50_50_1_1_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/Npowers100_50_1_1_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/Npowers200_50_1_1_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\\ \begin{subfigure}[b]{0.3466\textwidth}\input{graphs/stamps/Npowers100_100_1_1_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/Npowers200_100_1_1_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\begin{subfigure}[b]{0.3267\textwidth}\input{graphs/stamps/Npowers400_100_1_1_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\\ \begin{subfigure}[b]{\textwidth}\centering\input{graphs/stamps/lNpowers400_100_1_1_iid_0.4_iid_0.4_BN_.tex}\end{subfigure}\normalsize\caption{\label{NpowersiidBN111}Size-corrected power of unit-root tests as a function of $-h$ for varying sample sizes in the PANIC framework with i.i.d.\ factor innovations and i.i.d.\ idiosyncratic parts and $\sqrt{\omega^4/\phi^4}=1$. Based on \num{100000} replications.}\end{figure}
